PAUL: Procrustean Autoencoder for Unsupervised Lifting

Recent success in casting Non-rigid Structure from Motion (NRSfM) as an unsupervised deep learning problem has raised fundamental questions about what novelty in NRSfM prior could the deep learning offer. In this paper we advocate for a 3D deep auto-encoder framework to be used explicitly as the NRSfM prior. The framework is unique as: (i) it learns the 3D auto-encoder weights solely from 2D projected measurements, and (ii) it is Procrustean in that it jointly resolves the unknown rigid pose for each shape instance. We refer to this architecture as a Procustean Autoencoder for Unsupervised Lifting (PAUL), and demonstrate state-of-the-art performance across a number of benchmarks in comparison to recent innovations such as Deep NRSfM and C3PDO.

==> latex/sections/introduction_backup.tex <==

\section{Introduction}



In this paper we propose a new type of auto-encoder for modeling non-rigid 3D shapes. What makes this auto-encoder unique to current methods is: (i) it observes only 2D projected measurements of the non-rigid shape, (ii) it must automatically resolve the unknown rigid transformation for each projected shape instance, and (iii) the auto-encoder architecture is deep allowing for the compact of complex 3D shape object categories. We refer to our framework as \emph{Procustean Autoencoder for Unsupervised Lifting} (PAUL). Inferring non-rigid 3D structure from multiple unsynchronized 2D imaged observations is an ill-posed problem. Non-Rigid Structure from Motion (NR\SfM) methods approach the problem by introducing additional priors -- of particular note in this regards are low rank~\cite{dai2014simple,bregler2000recovering,akhter2009defense} and union of subspaces~\cite{kumar2016multi,zhu2014complex} methods. PAUL can be considered as a new framework for attacking such problems. 

Recently, NRSfM has seen a dramatic improvement in performance by recasting the problem as an unsupervised deep learning problem~\cite{c3dpo,cha2019unsupervised,park2020procrustean}. These 2D-3D \emph{lifting networks} have inherent advantages over classical NR\SfM as: (i) they are more easily scalable to larger datasets, and (ii) they allow fast feed-forward prediction once trained. These impressive results, however, can largely be attributed to the end-to-end reframing of the learning problem rather than any fundamental shift in the prior/constraints being enforced within the NRSfM solution. For example, both Cha~\etal~\cite{cha2019unsupervised} and Park~\etal~\cite{park2020procrustean} use a classical low rank to constraint on the recovered 3D shape. It is also well understood~\cite{ck19,zhu2014complex} that such low rank priors have poor performance when applied to more complex 3D shape variations. 

The NRSfM field has started to explore new non-rigid shape priors inspired by recent advances in deep learning. Kong \& Lucey~\cite{ck19} proposed the use of hierarchical sparsity to have a more expressive shape model while ensuring the inversion problem remains well conditioned. Although achieving significantly better results than state-of-the-art (at the time) the approach is limited by the somewhat adhoc approximations it employs so as to make the entire NRSfM solution realizable as a feed-forward lifting network -- which they refer to as Deep NRSfM. Such approximations hamper the interpretability of the method as the final network is a substantial departure from the actually proposed objective. We further argue that this departure from the true objective also comes at the cost of the overall effectiveness of the 2D-3D lifting solution. 

PAUL is considered unsupervised as it has to handle unknown depth, shape pose, and occlusions. Unlike Deep NRSfM~\cite{ck19}, the optimization process itself does not have to be realizable as a feed-forward network -- allowing for a solution that stays tightly coupled to the proposed mathematical objective. PAUL is advantageous over linear models commonly employed by previous methods, because the deeper auto-encoder is more capable of compressing complicated non-rigid 3D shapes. We also explore other alternate deep shape priors such as: decoder only and decoder + low-rank. Our empirical results demonstrate the fundamental importance of the auto-encoder architecture.   

\noindent \textbf{Contributions:} We make the following contributions:
\begin{itemize}
    \item We present an optimization objective for joint learning the 2D-3D lifting network and the Procrustean auto-encoder solely from 2D projected measurements.
    \item Demonstrate that a naiive implementation of PAUL through gradient descent would result in poor local minima -- so instead advocated for a bilevel optimization. This lower level problem can be efficiently solved by orthogonal-N-point (ONP) algorithms.
    \item Our method achieves  state-of-the-art performance across multiple benchmarks, and is empirically shown to be robust against the choice of hyper-parameters such as the dimension of the latent code space.  
\end{itemize}

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{latex/figs/teaser.pdf}
    \caption{PAUL learns to reconstruct 3D shapes aligned to a canonical frame, using 2D keypoint annotations only. }
    \label{fig:teaser}
\end{figure}

% Further, 


% Further, we demonstrate how this faithfulness to the objective is rewarded empirically by achieving state-of-the-art performance across multiple benchmarks. 




% Moreover, we note that an alternative approach with auto-decoder is applicable, but the constraint induced by auto-decoders is less sufficient compared to autoencoders due to missing the enforcement of the existence of an inverse mapping from 3D shape to latent code. Hitherto, additional prior constraints would be needed to supplement the use of auto-decoder. For example, Sidhu \etal~\cite{Sidhu2020} introduce extra priors such as spatial-temporal smoothness and encourage periodicity in trajectory, and consequently limited the use of their approach to dense reconstruction with sequential data. In this regard, Procrustean autoencoder is a more generic prior and is standalone sufficient to more challenging scenarios such as sparse reconstruction from non-sequential data.


% Despite the advantages of using autoencoders to model aligned 3D shapes, it is previously unclear how to apply to unsupervised 2D-3D lifting, due to the fact that autoencoders are typically learned with full supervision, while in the interest of this paper, the supervision is incomplete due to unknown depth and object poses as well as occlusions. Therefore, the main contributions of this paper are:


\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{latex/figs/pipeline.pdf}
    \caption{Caption}
    \label{fig:pipeline}
\end{figure*}



==> latex/sections/method_delete.tex <==
\begin{equation}
    \min_\theta \left\{\lambda \| \I_\text{input view}(\theta) - \I_\text{gt} \|_1 + \|D(\I_\text{novel view}(\theta))\|^2 \right\}
\end{equation}

\begin{equation}
        \min_{\theta_D} \|D(\I_\text{novel view}) - 1\|^2 + \|D(\I_\text{bg})\|^2
\end{equation}
